QoS-based Trust Evaluation for Data Services as a Black Box

This paper proposes a QoS-based trust evaluation model for black box data services. Under the black-box model, data services neither export (meta)-data about conditions in which they are deployed and collect and process data nor the quality of data they deliver. Therefore, the black-box model creates blind spots about the extent to which data providers can be trusted to be used to build target applications. The trust evaluation model for black box data services introduced in this paper originally combines QoS indicators, like service performance and data quality, to determine services trustworthiness. The paper also introduces DETECT: a Data sErvice as a black box Trust Evaluation arChitecTure, that validates our model. The trust model and its associated monitoring strategies have been assessed in experiments with representative case studies. The results demonstrate the feasibility and effectiveness of our solution.

==> oldAbstract.tex <==

%This  paper  proposes  a  QoS-based  trust  evaluationmodel  for  black  box  data  services.  Under  the  black  box  model services  neither  export  (meta)-data  about  conditions  in  which they  are  deployed  and  they  collect  and  process  data  nor  thequality of data they deliver to the user. This creates blind spots and  opens  up  questions  (services  avalability,  timeliness,  dataquality)  for  deteremining  to  which  extent  they  can  be  trustabledata providers and components to be used in target applications. Therefore, this paper proposes an approach for measuring trustcombining  QoS  indicators  including  service  performance  anddata  quality.  We  furthure  propose  DETECT:  a  Data  sErviceas   a  black   box   Trust  Evaluation   arChitecTure,  which   helpsimplementing  our  system  solution.  Through  experimentations,case  studies  are  used  to  demonstrate  the  feasibility  and  theeffectiveness  of  our  solution.

% This paper proposes a QoS-based trust evaluation model for data services available as black boxes that can be combined for answering user's queries. \genoveva{I do not think that we should refer to services coordination for answering queries. We can rather say: services that can be selected for collecting/querying data (with trust constraints.)} The black box paradigm \genoveva{black box is NOT a paradigm} creates blind spots and opens up multiple data service trust issues since they \genoveva{the subject in this sentence is "black box paradigm" and "they" refers to a service ..} neither export (meta)-data about conditions in which they collect and process data nor the quality of data they deliver to the user. The proposed trust measure is computed by combining QoS indicators, including service performance and data quality. Through experimentations, we demonstrate the feasibility and the effectiveness of our solution. 


==> oldIntro.tex <==
%ùwhere dealing with data services with potentially different trust levels can be an issue. 


%and thus, one cannot be sure about the fulfilment of the promised quality by the service provider.


%of data they manage (atomic data types like String, Integer, Float, and Composite data types like tuple, bag, and set).

%is often the result of expressing and evaluating queries that specify needs in terms of the data required and searching for potential data services that can provide them to the end-user according to specific conditions (freshness, availability etc.). 

%Therefore, looking up and selecting data services is crucial and  requires the consideration of the level of trustworthiness of the delivered data. 

%In general, the problem of providing “good” data services to clients and applications is a difficult problem that often depends on the application as well as the context and the current situation. In many cases, it is essential to provide users and applications with not only the necessary data through service selection, but also a trust index to determine how much we can trust the data delivered by these data services. Services' trust can be evaluated by combining QoS indicators including performance metrics and data quality metrics. 

 % main features characterise data services: first, the \textit{diversity of the available services} offering the same data under different QoS conditions and distinct data quality. Second, \textit{data services are represented as black boxes} as the only information they export is their API (Application Programming Interface) with methods and Input/Output parameters specifying what types of data they manage (atomic data types like String, Integer, Float, and Composite data types like tuple, bag, and set).  Third, the \textit{absence of meta-data} specifying the conditions under which data are delivered and their quality.  Indeed, they do not provide details on their backend, including how data are collected, how often data are updated, whether data are fresh (i.e. up-to-date), etc. Also, meta-data regarding the collected measures that a service provider monitors to determine the actual technical qualities of their services (availability, response time, security etc.) are not accessible to applications, and thus, one cannot be sure about the fulfilment of the promised quality by the service provider.
 
% In our work, we evaluate the quality of the accessed data which highly depends on the trustworthiness of the participating data service. This latter \genoveva{Services trust } can be evaluated by combining QoS indicators including performance metrics and data quality metrics. 
%To this end, estimating both service's performance and data quality for data services as a black box is challenging. 

%\textbf{When services are deployed on the cloud or elsewhere, they have an associated service level agreement (SLA) which includes clauses about the expected quality of service level (availability, response time, security etc.) }


 
%To this end, in order to evaluate the trust level of data services as black boxes: first, we check the fulfilment of the QoS offered by the different service providers by externally monitoring the performance of the used services, and second, we evaluate the quality of data. %\genoveva{We must avoir this type of wordy sentences.} 

% Therefore, the challenge is to propose protocols and strategies for evaluation data service as a black box trust level when there is no or little access to performance and data quality  meta-data.

% Let us introduce an e-health scenario proposed in the context of the project SUMMIT\footnote{\url{http://summit.imag.fr}} where dealing with data services with potentially different trust levels can be an issue. 


%Still, it would be advantageous if data services are tagged with a trust measure that could be updated recurrently. This measure indicates the trustworthiness data services and thus, would help choose the most relible amongst the available ones at a giving moment. Trust is based on the performance of the service and its data quality.
%Existing work has addressed the definition of metrics regarding service performance and data quality. Few works have addressed the evaluation of metric and trust index for black box data services, which motivates our proposal.

% .................................................................
%\subsection{Research Issues}
% .................................................................

% While many solutions have been used extensively to measure the trustworthiness level of services such as web services and cloud services using its QoS, including its performance \cite{a16,ref_journal15}, only a few efforts have been devoted for data trust evaluation, as pointed out the systematic review proposed by \cite{a5}. Besides, to the best of our knowledge, evaluating data quality having data services as black boxes from the client-side is still an open issue.

% As two critical solutions for successful data service selection, integrating QoS-based trustworthy service solutions and quality-based trustworthy data solutions can reinforce companies' decision-making, enhance data quality, and QoS of data services.  Thus, how to seamlessly integrate these two domains is an urgent research task. Based on the identified features of service-based data integration and the motivated trust needs through our scenario, we believe there is still a gap related to the definition of a trust model for data services and the black box paradigm. Such gaps raise the following research problems (RPs). 
% \newline
% (RP1) What is the appropriate model for describing data services QoS-based trust? How to define both service performance metrics and data quality metrics to be used in the trust evaluation process? 
% \newline
% (RP2) How to collect the necessary information for this trust evaluation model?  
% \newline
%(RP3) While creating a prototype to validate the proposed contribution that aims at addressing the first research problem (RP1), potential issues can emerge during the implementation phase. Moreover, analyzing the proposal’s feasibility and practicability demonstrates whether the solution can be used in practice. Therefore, we consider the following research question: Is the proposed solution feasible and implementable? 

%\genoveva{Do we answer all these questions in the paper? A sentence here saying which are the questions addressed in the paper and how do we manage to answer them can be interesting. Then in the section experimentation we can enumerate these questions and discuss results.}

==> oldRelatedWork.tex <==
%----------------------------------
\section{Related Work}\label{sec:related}
%----------------------------------
%
Service trust evaluation has been widely addressed by research works targeting different service-based environments, including SOA, web services, cloud services etc.  

    % . . . . . . . . . . . . . . . . . . . . . . .  . . . . ..
    \subsection{Trustworthy Services}
    % . . . . . . . . . . . . . . . . . . . . . . .  . . . . ..
    %We have studied research papers addressing service trust evaluation solutions. This study reveals that 
    Existing service trust evaluation solutions differ in the type of the adopted trust assessment model (fuzzy models \cite{a7,a8,a9}, probabilistic models \cite{a10}, machine learning models \cite{a11,a12,a13}, multi-criteria decision-making models (MCDM) \cite{a14,a15} and classical mathematical models such as weighted-addition \cite{a16}).
    The service trust evaluation can be subjective \cite{a17,a18}, objective\cite{a16,a19} or hybrid\cite{a20,p15} (subjective + objective). Subjective evaluation relies on user preferences and feedback about the service usage for evaluating trust. Users' feedback may be delivered as a quantitative opinion or as a qualitative opinion in textual form. 
    The objective evaluation uses measurable information in the trust level evaluation such as the service capacities, service capabilities and service performance\cite{a5}. Note that users' subjective feedback may be influenced by several factors and may exhibit significant variations in the evaluation of the same service from one user to another. Besides, there is no guarantee of users' honesty. 
    
    %For these reasons, we are only interested in the objective trust evaluation.
    
    %In our previous work \cite{a5}, we have studied research papers addressing cloud service trust evaluation. Results show that various efforts already exist to study different trust aspects of cloud services \cite{p11,ref_journal15,ref_journal16,ref_journal17}.This study found that service trust level can be computed using different factors, including service performance, service capacity, and service capability. 
    %However, 
    Performance can be measured using several metrics: service availability, service response time, service reliability, service security and so on.
    Objective service trust evaluation mainly uses service performance\cite{a5} as a reference measure which is also considered a significant criterion for selecting services. Services performance is computed through SLA monitoring, where information is collected from previous experiences using a service and is used to measure the degree of SLA fulfilment\cite{ref_proc4}. If the SLA is satisfied, then the service is considered trustworthy. 
    
    %More details can be found in \emph{autocite}
    
    %Xiaoyong et al.  \cite{ref_journal14}: Availability, Average response time, average task success ratio, and the number of malicious access.
    
     %Chiregi et al. \cite{ref_journal16} Availability, Reliability (task success ratio), data integrity (includes privacy and data accuracy)
     
     % Singh et al. \cite{ref_journal17} Data processing accuracy, Data privacy, Data storage success, data transmission (\% of success), and data security. Availability, Reliability, Turnaround time and service use factor of the service (related  to  the number of users that uses the service)
      
     % Mrabet et al. (2016) \cite {p11}: \textbf{Q:} How to evaluate cloud services trust taking into consideration objective and subjective evidence? How to make sure that subjective evidence is correct. \textbf{Objective:} Design a new trust evaluation approach that leverages the correlation between QoS attribute capable of deterring unreasonable/false feedback. \textbf{approach}: Authors take into account the possible correlations between QoS attributes and classify them into dependent and independent attributes. Thus, filtering unreasonable assessment reports \textbf{Performance:} Availability (\% accepted requests), Reliability (\%  requests  successfully  completed), Time efficiency, Data integrity
      
    %\item 
        % . . . . . . . . . . . . . . . . . . . . . . .  . . . . ..
    \subsection{Trustworthy Data}
        % . . . . . . . . . . . . . . . . . . . . . . .  . . . . ..
        
     Data similarity and data provenance are the two mostly features used to evaluate data trust. Similarity-based solutions considers that the  more similar the data  values  from the same event are , the more likely the data is correct and therefore trustworthy. Provenance-based solutions considers that data with good provenance is more likely to be trustworthy.
     

     %
     In addition, several studies focus on the definition of metrics for data quality evaluation\cite{p16,p18}. 
     %without explaining ways in which the required information for this evaluation are retrieved. 
     Authors assume that this information is already exported by data providers as evidence of honesty, or that it is accessible. 
     %
     %In the context of data services as a black box, this type of information can't be retrieved and is not provided by the service.
    %
    Authors in \cite{p6} evaluate data quality and data trustworthiness using the web provenance information.  In their approach, they collect provenance information and evaluate it for data quality evaluation.
    %Provenance information represents the creation of a data item and information about the entities who made data accessible on the web. 
    %They further demonstrate their generic method by evaluating data timeliness to reflect how up-to-date the data is. 
    %In this paper, some pieces of provenance information can be recorded by the system; for other pieces the system relies on meta-data found on the web.
    %based on their model they identify options to obtain provenance information and they raise open questions concerning the publication of provenance-related metadata for linked data on the Web.
    
    Works proposed in  \cite{p8,p9} evaluate location-based data trustworthiness using data provenance.  The approach uses GPS data to trace people's location to generate meta-data about provenance available and accessible. Data provenance is completed using  evidence from different sources and adopting the data similarity approach. 
    %(similar data are considered as supportive to each other).
    %Their trust model is based on several factors namely \textit{Data similarity} (Similar items are considered as supportive to each other), \textit{Path similarity} (Affects the importance of supports obtained from similar data), \textit{Data conflict} (Refers to inconsistent descriptions about the same entity or event.) and \textit{Data deduction} (trustworthiness of a knowledge item also depends on the trustworthiness of information used to generate it). 
   
    
    In \cite{p10,p11}, authors propose a systematic method for assessing the trustworthiness of data items in sensor networks. Trust score is computed using data provenance and their values based on their similarity "the more similar values for the same event, the higher the trust scores". In this approach, the trust score of the data affects the trust score of the network nodes that created and manipulated the data and vice-versa.
    
     
    The work in \cite{p20} proposes a novel data provenance trusted model in cloud computing. Authors believe that to establish trust with users, cloud service providers should consider providing trust information such as provenance record. Based on this hypothesis, meta-data about provenance is provided by a cloud provider.
    
    The work in \cite{p21} proposes trustworthy and secure management of provenance in cloud computing. It captures the complete provenance of any entities in the cloud without trusting cloud providers. They do not take into consideration the fact that provenance is meta-data hidden behind the service's API.
       
       
   Neumaeir et al. in \cite{p16} introduce measures for assessing data freshness in open data portals. The challenge is to determine the reliability of data update frequency, considering that there is no proof that this information is correct or respected.
    In their approach, first, they learn the change history of a data source and then apply a heuristic to estimate how up-to-date a data source is. Three ways to collect change information are discussed: comparison-based (empirical distribution, Poisson process or Markov chain approach), age-based (empirical distribution, Poisson process) and push-based.  They estimate data freshness using the history of information changes, assuming that resources update frequency is not available.

    %empirical distribution:
    %%comparison-based: a constant sampling interval is used and check if there are any changes
    
    %%age based: using the intervals between the observed last-modified time
    
    %poisson process: authors assume that a data item changes by a Poisson process since “a Poisson process is often used to model a sequence of random events that happen independently with a fixed rate over time
    
   
   In \cite{p18,p19}, authors propose a framework for evaluating data freshness in a data integration system (DIS). They define how data freshness value changes in DIS for data moving from data sources to users. Their work evaluates the evolution of data freshness using graphs representing the integration workflows in a controlled environment. They do not need to worry about the existence or not of meta-data about data provenance.
   
    
% . . . . . . . . . . . . . . . . . . . . . . .  . . . . ..
\subsection{Trustworthy Data Services: Discussion}
% . . . . . . . . . . . . . . . . . . . . . . .  . . . . ..
    Existing work proposes models to define data quality metrics and performance metrics and strategies to capture data %\genoveva{metrics? data?} for evaluating these metrics.
    %services performance 
    %\genoveva{This sentence is circular, models to define performance metrics for evaluating performance ???}. 
     \genoveva{The final discussion must argue about the metrics used for measuring trust, whether they are "formally" defined with the same formulas, the strategies adopted for collecting, aggregating and combining them to estimate trust.}
\senda{I think like you said, it is better to focus on data service trust evaluation metrics and data and why papers don't propose a trust model for data services and talk less about the black box as we do not tackle the observation protocol in this paper. I am going to reformulate this discussion tomorrow morning}
The general assumption in current work is that service providers may export service execution measures or data quality observations as a proof of good will to cooperate and to show that they provide "good" services. %The behaviour of the services is observed and collected in histories or logs that are used to compute technical metrics needed for "estimating" services performance and trust. 
While service providers perform services' metrology with full control on services' execution environement and the data they manage, service consumers can only use their non-professional day-to-day experience and clauses in Service Level Agreements (SLA) to decide whether or not they can trust a given service.
As the access to data services has been democratised, service consumers need
%full control and 
quantitative evidence about the real QoS and the quality of data they are consuming. However, for technical and privacy reasons, quality metrics are not exported in free access modes outside deployment platforms and providers. 
Still, clients are looking for alternatives to evaluate the trust level of both services and data to use it to choose services for building information systems and retrieving data.
To the best of our knowledge, measuring (data) quality and QoS metrics of black box data services is yet to come. 
%In fact, information in those works are mostly available as they are either included in meta-data or provided by the data source in question. For partially missing information, methods are proposed to estimate it using past history. 
    
   % Nevertheless, taking into consideration the black box model 
    %\genoveva{black box is neither a "baradigm" not a paradigm}
    ,
 %   they fail to provide methods for the capturing of the necessary information for the measuring of data quality metrics \genoveva{they do not consider measuring data quality of black box data services}.  \genoveva{???}
    %In the context of data services as a black box, this type of information can't be retrieved and is not provided by the service.
    %
   % \genoveva{Why is data quality not considered? Is existing work considering services that do not provide data? Are they adopting specific hypothesis or is their definition of trust incomplete?}

 %In our work, we use metadata about data quality to assess the trustworthiness level of data.  To the best of our knowledge, there are no solutions in the literature where data quality is used to assess data trust level. 
  
   % \genoveva{Here discussion about the way trust models are incomplete/limited for estimating trust level for data services as black boxes.}

